Dynamic Slimmable Networks for Efficient Speech Separation

Recent progress in speech separation has been largely driven by advances in deep neural networks, yet their high computational and memory requirements hinder deployment on resource-constrained devices. A significant inefficiency in conventional systems arises from using static network architectures that maintain constant computational complexity across all input segments, regardless of their characteristics. This approach is sub-optimal for simpler segments that do not require intensive processing, such as silence or non-overlapping speech. To address this limitation, we propose a dynamic slimmable network (DSN) for speech separation that adaptively adjusts its computational complexity based on the input signal. The DSN combines a slimmable network, which can operate at different network widths, with a lightweight gating module that dynamically determines the required width by analyzing the local input characteristics. To balance performance and efficiency, we introduce a signal-dependent complexity loss that penalizes unnecessary computation based on segmental reconstruction error. Experiments on clean and noisy two-speaker mixtures from the WSJ0-2mix and WHAM! datasets show that the DSN achieves a better performance-efficiency trade-off than individually trained static networks of different sizes.

==> tables/robustness.tex <==

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.7}
    \caption{Performance of the \acp{DSN} under internal and external gating, reported in terms of \ac{SI-SDR}i (dB). For internal gating, the average utilization is shown in parentheses  next to the \ac{SI-SDR}i scores. The \acp{DSN} results are shown for models trained with $\alpha = 1.0$, $w_t^{\text{SD}}$, $a = 0.05$, and $b = 20$.}
    \label{tab:robustness}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lccccc@{}}
    \toprule
    \textbf{Model} & \textbf{Dropout} & \multicolumn{1}{c}{\textbf{Internal Gating}} & \multicolumn{3}{c}{\textbf{External Gating}} \\
                   &                  &           & $U_t{=}0.125$ & $U_t{=}0.5$ & $U_t{=}1.0$ \\ \midrule
    Static & - & -     & 16.1 & 19.2 & 20.3 \\ 
    DSN ($\mathcal{U}{=}\{0.125, 1.0\}$)         & \xmark & 19.7 (0.55) & \phantom{0}7.4 & -    & 16.6 \\
    DSN ($\mathcal{U}{=}\{0.125, 1.0\}$)         & \cmark & 19.3 (0.55) & 15.3 & -    & 19.9 \\
    DSN ($\mathcal{U}{=}\{0.125, 0.5, 1.0\}$)    & \xmark & 19.2 (0.54) & \phantom{0}8.9 & 15.3 & 13.0 \\
    DSN ($\mathcal{U}{=}\{0.125, 0.5, 1.0\}$)    & \cmark & 19.2 (0.49) & 15.0 & 18.6 & 19.5 \\ 
    \bottomrule  
    \end{tabular}%
    }
\end{table}
